Revisiting Poisson-disk Subsampling for Massive Point Cloud Decimation

Scanning devices often produce point clouds exhibiting highly uneven distributions of point samples across the surfaces being captured. Different point cloud subsampling techniques have been proposed to generate more evenly distributed samples. Poisson-disk sampling approaches assign each sample a cost value so that subsampling reduces to sorting the samples by cost and then removing the desired ratio of samples with the highest cost. Unfortunately, these approaches compute the sample cost using pairwise distances of the points within a constant search radius, which is very costly for massive point clouds with uneven densities. In this paper, we revisit Poisson-disk sampling for point clouds. Instead of optimizing for equal densities, we propose to maximize the distance to the closest point, which is equivalent to estimating the local point density as a value inversely proportional to this distance. This algorithm can be efficiently implemented using k nearest-neighbors searches. Besides a kd-tree, our algorithm also uses a voxelization to speed up the searches required to compute per-sample costs. We propose a new strategy to minimize cost updates that is amenable for out-of-core operation. We demonstrate the benefits of our approach in terms of performance, scalability, and output quality. We also discuss extensions based on adding orientation-based and color-based terms to the cost function.

==> figures/figure2-carlos.tex <==
\begin{figure*}[!htb]
\centering
\begin{tabular*}{\linewidth}{cccccc}  % left bottom right top
    \rotatebox[origin=c]{90}{Top Face} &
    \raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth,trim=100 100 900 900, clip]{cube/cube_452k_top_den.png}} &
    \raisebox{-0.5\height}{\includegraphics[trim=100 100 900 900, clip,width=0.18\linewidth]{cube/cube_452k_y00-10_top_points.png}} &
    \raisebox{-0.5\height}{\includegraphics[trim=100 100 900 900, clip,width=0.18\linewidth]{cube/cube_452k_y35-10_top_points.png}} &
    \raisebox{-0.5\height}{\includegraphics[trim=100 100 900 900, clip,width=0.18\linewidth]{cube/cube_452k_y65-10_top_points.png}} &
    \raisebox{-0.5\height}{\includegraphics[trim=100 100 900 900, clip,width=0.18\linewidth]{cube/cube_452k_y100-10_top_points.png}} 
    \\
    & Original Cloud & Yuksel ($\beta=0$) & Yuksel ($\beta=0.35$) & Yuksel ($\beta=0.65$) & Yuksel ($\beta=1$)
    \\
    \rotatebox[origin=c]{90}{Top Face} &
    \raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{cube/cube_452k_d10_top_points.png}} &
    \raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{cube/cube_452k_c10_top_points.png}} &
    \raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{cube/cube_452k_v10-10-1_top_points.png}} &
    \raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{cube/cube_452k_v10-10-3_top_points.png}} &
    \raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{cube/cube_452k_v10-10-6_top_points.png}} 
    \\
    & Dart Throwing & Corsini & Ours ($k=1$) & Ours ($k=3$) & Ours ($k=6$) 
    \\
    \rotatebox[origin=c]{90}{Right Face} &
    \raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{cube/cube_452k_right_den.png}} &
    \raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{cube/cube_452k_y00-10_right_points.png}} &
    \raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{cube/cube_452k_y35-10_right_points.png}} &
    \raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{cube/cube_452k_y65-10_right_points.png}} &
    \raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{cube/cube_452k_y100-10_right_points.png}} 
    \\
    & Original Cloud & Yuksel ($\beta=0$) & Yuksel ($\beta=0.35$) & Yuksel ($\beta=0.65$) & Yuksel ($\beta=1$)
    \\
    \rotatebox[origin=c]{90}{Right Face} &
    \raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{cube/cube_452k_d10_right_points.png}} &
    \raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{cube/cube_452k_c10_right_points.png}} &
    \raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{cube/cube_452k_v10-10-1_right_points.png}} &
    \raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{cube/cube_452k_v10-10-3_right_points.png}} &
    \raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{cube/cube_452k_v10-10-6_right_points.png}} 
    \\
    & Dart Throwing & Corsini & Ours ($k=1$) & Ours ($k=3$) & Ours ($k=6$)
    \\
    \rotatebox[origin=c]{90}{Statistics} &
    \raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{cube/cube_452k_legend.png}} &
    \raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{cube/cube_452k_y00-10_area.png}} &
    \raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{cube/cube_452k_y35-10_area.png}} &
    \raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{cube/cube_452k_y65-10_area.png}} &
    \raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{cube/cube_452k_y100-10_area.png}} 
    \\
    & Legend & Yuksel ($\beta=0$) & Yuksel ($\beta=0.35$) & Yuksel ($\beta=0.65$) & Yuksel ($\beta=1$)
    \\
    \rotatebox[origin=c]{90}{Statistics} &
    \raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{cube/cube_452k_d10_area.png}} &
    \raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{cube/cube_452k_c10_area.png}} &
    \raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{cube/cube_452k_v10-10-1_area.png}} &
    \raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{cube/cube_452k_v10-10-3_area.png}} &
    \raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{cube/cube_452k_v10-10-6_area.png}} 
    \\
    & Dart Throwing & Corsini & Ours ($k=1$) & Ours ($k=3$) & Ours ($k=6$)
\end{tabular*}
\caption{\label{fig:c4f2} Analysis of the simplifications of a point cloud of a cube using different algorithms. The original cloud was generated simulating 80 LiDAR scans around a cubic mesh. The first four rows show the results on two faces of the cloud (top, right) compared to the original cloud colored according to the local point density. The last two rows show, for each algorithm, the distribution of local point densities with increasing neighborhood radius. }
\end{figure*}

==> figures/figure2.tex <==
\begin{figure}[!htb]
\centering
   \begin{subfigure}[t]{0.35\linewidth}
    \includegraphics[width=1\linewidth]{c4f2i1a}
    \caption{Cloud simplified using Yuksel~\cite{yuksel2015}.}
    \label{fig:c4f2i1}
  \end{subfigure}
    \hspace{1cm}
  \begin{subfigure}[t]{0.35\linewidth}
    \includegraphics[width=1\linewidth]{c4f2i2a}
    \caption{Cloud simplified using our approach.}
   \label{fig:c4f2i2}
  \end{subfigure}
\caption{ Yuksel~\cite{yuksel2015}'s approach \textit{(a)} produces small clusters, but these are well-distributed across the space.
Our approach \textit{(b)} maximizes the minimum separation between point samples.  
} 
\label{fig:c4f2}
\end{figure}

==> figures/figure3.tex <==
\begin{figure*}[!htb]
\centering
    \includegraphics[width=0.12\linewidth]{c4f4i2i1}
    \includegraphics[width=0.12\linewidth]{c4f4i2i2}
    \includegraphics[width=0.12\linewidth]{c4f4i2i3}
    \includegraphics[width=0.12\linewidth]{c4f4i2i5}
    \includegraphics[width=0.12\linewidth]{c4f4i2i4}
    \includegraphics[width=0.12\linewidth]{c4f4i2i6}
    \includegraphics[width=0.12\linewidth]{c4f4i2i7}
    \includegraphics[width=0.12\linewidth]{c4f4i2i8}

    \includegraphics[width=0.12\linewidth]{c4f4i3i1}
    \includegraphics[width=0.12\linewidth]{c4f4i3i2}
    \includegraphics[width=0.12\linewidth]{c4f4i3i3}
    \includegraphics[width=0.12\linewidth]{c4f4i3i5}
    \includegraphics[width=0.12\linewidth]{c4f4i3i4}
    \includegraphics[width=0.12\linewidth]{c4f4i3i6}
    \includegraphics[width=0.12\linewidth]{c4f4i3i7}
    \includegraphics[width=0.12\linewidth]{c4f4i3i8}

    \includegraphics[width=0.12\linewidth]{c4f4i5i1}
    \includegraphics[width=0.12\linewidth]{c4f4i5i2}
    \includegraphics[width=0.12\linewidth]{c4f4i5i3}
    \includegraphics[width=0.12\linewidth]{c4f4i5i5}
    \includegraphics[width=0.12\linewidth]{c4f4i5i4}
    \includegraphics[width=0.12\linewidth]{c4f4i5i6}
    \includegraphics[width=0.12\linewidth]{c4f4i5i7}
    \includegraphics[width=0.12\linewidth]{c4f4i5i8}

    \includegraphics[width=0.12\linewidth]{c4f4i7i1}
    \includegraphics[width=0.12\linewidth]{c4f4i7i2}
    \includegraphics[width=0.12\linewidth]{c4f4i7i3}
    \includegraphics[width=0.12\linewidth]{c4f4i7i5}
    \includegraphics[width=0.12\linewidth]{c4f4i7i4}
    \includegraphics[width=0.12\linewidth]{c4f4i7i6}
    \includegraphics[width=0.12\linewidth]{c4f4i7i7}
    \includegraphics[width=0.12\linewidth]{c4f4i7i8}

    \includegraphics[width=0.12\linewidth]{c4f4i13i1}
    \includegraphics[width=0.12\linewidth]{c4f4i13i2}
    \includegraphics[width=0.12\linewidth]{c4f4i13i3}
    \includegraphics[width=0.12\linewidth]{c4f4i13i5}
    \includegraphics[width=0.12\linewidth]{c4f4i13i4}
    \includegraphics[width=0.12\linewidth]{c4f4i13i6}
    \includegraphics[width=0.12\linewidth]{c4f4i13i7}
    \includegraphics[width=0.12\linewidth]{c4f4i13i8}
    
    \includegraphics[width=0.12\linewidth]{c4f4i14i1}
    \includegraphics[width=0.12\linewidth]{c4f4i14i2}
    \includegraphics[width=0.12\linewidth]{c4f4i14i3}
    \includegraphics[width=0.12\linewidth]{c4f4i14i5}
    \includegraphics[width=0.12\linewidth]{c4f4i14i4}
    \includegraphics[width=0.12\linewidth]{c4f4i14i6}
    \includegraphics[width=0.12\linewidth]{c4f4i14i7}
    \includegraphics[width=0.12\linewidth]{c4f4i14i8}
 
    \includegraphics[width=0.12\linewidth]{c4f4i15i1}
    \includegraphics[width=0.12\linewidth]{c4f4i15i2}
    \includegraphics[width=0.12\linewidth]{c4f4i15i3}
    \includegraphics[width=0.12\linewidth]{c4f4i15i5}
    \includegraphics[width=0.12\linewidth]{c4f4i15i4}
    \includegraphics[width=0.12\linewidth]{c4f4i15i6}
    \includegraphics[width=0.12\linewidth]{c4f4i15i7}
    \includegraphics[width=0.12\linewidth]{c4f4i15i8}
 
    \includegraphics[width=0.12\linewidth]{c4f4i17i1}
    \includegraphics[width=0.12\linewidth]{c4f4i17i2}
    \includegraphics[width=0.12\linewidth]{c4f4i17i3}
    \includegraphics[width=0.12\linewidth]{c4f4i17i5}
    \includegraphics[width=0.12\linewidth]{c4f4i17i4}
    \includegraphics[width=0.12\linewidth]{c4f4i17i6}
    \includegraphics[width=0.12\linewidth]{c4f4i17i7}
    \includegraphics[width=0.12\linewidth]{c4f4i17i8}
    
\caption{Evaluation of our results on synthetic data. From left to right: \textbf{(1)} Input polygonal models. \textbf{(2)} Synthetic point clouds reproducing LiDAR data. Scan locations are represented by blue spheres. Color represents the local point density deviation with respect to the average density, using a logarithmic scale: \textit{white} (0), \textit{yellow} ($10^3$) and \textit{red} ($10^6$). \textbf{(3)} Our sub-sampled output ($\lambda = 0.1$), with color also encoding local density deviation. Notice that values are much smaller, meaning our densities are much more homogeneous. \textbf{(4)} Distribution of local density deviations on the original (\textit{red} curves) and the sub-sampled clouds (\textit{blue} curves). Notice that the improvement spans one to three orders of magnitude. The curve outline color also encodes local density deviation.
\textbf{(5)} Running time comparison between our method (\textit{blue} curves), Yuksel~\cite{yuksel2015} (\textit{red} curves) and Corsini et al.~\cite{corsini2012} (\textit{green} curves). Our running times include out-of-core operations while the other two are executed in-core. Despite this I/O overhead, in most cases our algorithm is faster than \cite{yuksel2015}, specially on those models with very dense regions, where performing radius search is very inefficient. \cite{corsini2012} is generally faster but it is hard to compare as it rarely meets the target number of samples. \textbf{(6)}, \textbf{(7)} and \textbf{(8)} show the distribution of distances from a point to its \textit{i}-th closest neighbor. \cite{yuksel2015} and \cite{corsini2012} lead to smaller distances to the closest neighbor, namely Poisson disk samples with smaller radius. \cite{yuksel2015} also yields more irregular distributions (specially when the closest and second closest neighbor are considered). Instead, our curves have a constant shift. This means neighbors are placed at regular intervals, which intuitively indicates we are producing uniformly distributed samples. Similarly, \cite{corsini2012} curves are also quite well-distributed. Their smaller distance to the closest neighbor can be explained by their algorithm not being able to reach the target decimation factor. For most models it returned a much larger (and denser) cloud than requested. }
\label{fig:c4f4}
\end{figure*}


==> figures/figure4.tex <==
\begin{figure}[tb]
\centering
    \includegraphics[width=0.24\linewidth]{ccours}
    \includegraphics[width=0.24\linewidth]{ccrand}
    \includegraphics[width=0.24\linewidth]{errours}
    \includegraphics[width=0.24\linewidth]{errrand}
\caption{From left to right: (a) distribution of samples selected by our algorithm on a roughly planar surface (close-up from our 10\% decimation of the Apse B model). Some apparently tight point pairs are actually far apart in 3D, due to some samples from distant scans being off the surface; (b) samples selected by random sampling; (c) error measured as the distance from each original point to its closest point in our decimated sample; (d) the same error in the random sample.}
\label{fig:err}
\end{figure}

==> figures/figure5.tex <==
\begin{figure}[!htb]
\centering
    \includegraphics[width=0.49\linewidth]{c4f3i1}
    \includegraphics[width=0.49\linewidth]{c4f3i2}
    
    \includegraphics[width=0.49\linewidth]{c4f3i3}
    \includegraphics[width=0.49\linewidth]{c4f3i4}
\caption{ Running times for real \textbf{(top)} and synthetic \textbf{(bottom)} datasets. The \textbf{(top)} row shows the times for simplifying from 100\% to 10\% of the original samples \textbf{(left)} and for simplifying from 10\% to 1\% of the original samples \textbf{(right)} for the real models Apse A (297 Mpts), Market (372 Mpts), Abse B (557 Mpts), Church (1026 Mpts), Chapel Outside (1191 Mpts), Chapel Inside (1213 Mpts) and Museum (1250 Mpts). On the \textbf{(bottom)} row we show the times for simplifying from 100\% to  10\% of the original samples \textbf{(left)} and from 100\% to 1\% of the original samples \textbf{(right)}for the synthetic models apartment (676 Kpts), baidinh (470 Kpts), bungalow (662 Kpts), cabin (778 Kpts), cathedral (437 Kpts), chapel (538 Kpts), church (429 Kpts), cottage (654 Kpts), highrise (659 Kpts), house (512 Kpts), japanese (552 Kpts), mansion (614 Kpts), monastery (550 Kpts), mosque (514 Kpts), oldhouse (804 Kpts), petersdom (397 Kpts), pisa (457 Kpts) and sanfrancisco (690 Kpts). We have found experimentally that each decimation iteration roughly removes half of the samples to the target (the first iterations are represented as 
horizontal dashed lines). E.g. when aiming to a 10\% of the original samples, the first iteration will remove 45\% of those, the second 22.5\% and so on. We have also found that the execution does not only depend on the number of points but also on their distribution, for instance Museum (1250 Mpts) took few time than Chapel Inside (1213 Mpts). }
\label{fig:c4f3}
\end{figure}


==> figures/figure6.tex <==
\begin{figure*}[!htb]
\centering

    \includegraphics[width=0.19\linewidth]{c4f5i2i1}
    \includegraphics[width=0.19\linewidth]{c4f5i2i2}
    \includegraphics[width=0.19\linewidth]{c4f5i2i3}
    \includegraphics[width=0.19\linewidth]{c4f5i2i4}
    \includegraphics[width=0.19\linewidth]{c4f5i2i5}
    
    \includegraphics[width=0.19\linewidth]{c4f5i4i1}
    \includegraphics[width=0.19\linewidth]{c4f5i4i2}
    \includegraphics[width=0.19\linewidth]{c4f5i4i3}
    \includegraphics[width=0.19\linewidth]{c4f5i4i4}
    \includegraphics[width=0.19\linewidth]{c4f5i4i5}
    
    \includegraphics[width=0.19\linewidth]{c4f5i3i1}
    \includegraphics[width=0.19\linewidth]{c4f5i3i2}
    \includegraphics[width=0.19\linewidth]{c4f5i3i3}
    \includegraphics[width=0.19\linewidth]{c4f5i3i4}
    \includegraphics[width=0.19\linewidth]{c4f5i3i5}
    
    \includegraphics[width=0.19\linewidth]{c4f5i1i1}
    \includegraphics[width=0.19\linewidth]{c4f5i1i2}
    \includegraphics[width=0.19\linewidth]{c4f5i1i3}
    \includegraphics[width=0.19\linewidth]{c4f5i1i4}
    \includegraphics[width=0.19\linewidth]{c4f5i1i5}
    
    \includegraphics[width=0.19\linewidth]{c4f5i5i1}
    \includegraphics[width=0.19\linewidth]{c4f5i5i2}
    \includegraphics[width=0.19\linewidth]{c4f5i5i3}
    \includegraphics[width=0.19\linewidth]{c4f5i5i4}
    \includegraphics[width=0.19\linewidth]{c4f5i5i5}
    
    \includegraphics[width=0.19\linewidth]{c4f5i6i1}
    \includegraphics[width=0.19\linewidth]{c4f5i6i2}
    \includegraphics[width=0.19\linewidth]{c4f5i6i3}
    \includegraphics[width=0.19\linewidth]{c4f5i6i4}
    \includegraphics[width=0.19\linewidth]{c4f5i6i5}
    
    \includegraphics[width=0.19\linewidth]{c4f5i7i1}
    \includegraphics[width=0.19\linewidth]{c4f5i7i2}
    \includegraphics[width=0.19\linewidth]{c4f5i7i3}
    \includegraphics[width=0.19\linewidth]{c4f5i7i4}
    \includegraphics[width=0.19\linewidth]{c4f5i7i5}
\caption{Evaluation of our results on real data. From top to bottom:  Apse A (297 Mpts), Market (372 Mpts), Abse B (557 Mpts), Church (1026 Mpts), Chapel Outside (1191 Mpts), Chapel Inside (1213 Mpts) and Museum (1250 Mpts). From left to right: \textbf{(1)} Cloud rendered using phong-shading. Scan locations are represented by blue spheres. \textbf{(2)}, \textbf{(3)} and \textbf{(4)} Simplified clouds (10\%, 1\% and 0.1\% of the original samples). Color represents the local point density deviation with respect to the average density, using a logarithmic scale and \textit{white} (0), \textit{yellow} ($10^3$) and \textit{red} ($10^6$) interpolated colors.
\textbf{(5)} shows the distribution of local density deviations on the original (rightmost curve) and the three sub-sampled clouds.}
\label{fig:c4f5}
\end{figure*}


==> figures/figure9.tex <==
\begin{figure}[!htb]
\centering
   \begin{subfigure}[t]{0.24\linewidth}
    \includegraphics[width=1\linewidth]{c4f7i1i1}
    \caption{}
    \label{fig:c4f9i1i1}
  \end{subfigure}
  \begin{subfigure}[t]{0.24\linewidth}
    \includegraphics[width=1\linewidth]{c4f7i1i2}
    \caption{}
   \label{fig:c4f9i1i2}
  \end{subfigure}
  \begin{subfigure}[t]{0.24\linewidth}
    \includegraphics[width=1\linewidth]{c4f7i1i3}
    \caption{}
   \label{fig:c4f9i1i3}
  \end{subfigure}
  \begin{subfigure}[t]{0.24\linewidth}
    \includegraphics[width=1\linewidth]{c4f7i1i4}
    \caption{}
   \label{fig:c4f9i1i4}
  \end{subfigure}

  \begin{subfigure}[t]{0.24\linewidth}
    \includegraphics[width=1\linewidth]{c4f7i2i1}
    \caption{}
    \label{fig:c4f9i2i1}
  \end{subfigure}
  \begin{subfigure}[t]{0.24\linewidth}
    \includegraphics[width=1\linewidth]{c4f7i2i2}
    \caption{}
   \label{fig:c4f9i2i2}
  \end{subfigure}
  \begin{subfigure}[t]{0.24\linewidth}
    \includegraphics[width=1\linewidth]{c4f7i2i3}
    \caption{}
   \label{fig:c4f9i2i3}
  \end{subfigure}
  \begin{subfigure}[t]{0.24\linewidth}
    \includegraphics[width=1\linewidth]{c4f7i2i4}
    \caption{}
   \label{fig:c4f9i2i4}
  \end{subfigure} 
  
  \begin{subfigure}[t]{0.24\linewidth}
    \includegraphics[width=1\linewidth]{c4f7i3i1}
    \caption{}
    \label{fig:c4f9i3i1}
  \end{subfigure}
  \begin{subfigure}[t]{0.24\linewidth}
    \includegraphics[width=1\linewidth]{c4f7i3i2}
    \caption{}
   \label{fig:c4f9i3i2}
  \end{subfigure}
  \begin{subfigure}[t]{0.24\linewidth}
    \includegraphics[width=1\linewidth]{c4f7i3i3}
    \caption{}
   \label{fig:c4f9i3i3}
  \end{subfigure}
  \begin{subfigure}[t]{0.24\linewidth}
    \includegraphics[width=1\linewidth]{c4f7i3i4}
    \caption{}
   \label{fig:c4f9i3}
  \end{subfigure}
  
%  \begin{subfigure}[t]{0.24\linewidth}
%    \includegraphics[width=1\linewidth]{c4f7i4i1}
%    \caption{}
%    \label{fig:c4f9i4i1}
%  \end{subfigure}
%  \begin{subfigure}[t]{0.24\linewidth}
%    \includegraphics[width=1\linewidth]{c4f7i4i2}
%    \caption{}
%   \label{fig:c4f9i4i2}
%  \end{subfigure}
%  \begin{subfigure}[t]{0.24\linewidth}
%    \includegraphics[width=1\linewidth]{c4f7i4i3}
%    \caption{}
%   \label{fig:c4f9i4i3}
%  \end{subfigure}
%  \begin{subfigure}[t]{0.24\linewidth}
%    \includegraphics[width=1\linewidth]{c4f7i4i4}
%    \caption{}
%   \label{fig:c4f9i4i4}
%  \end{subfigure}
  
  \begin{subfigure}[t]{0.24\linewidth}
    \includegraphics[width=1\linewidth]{c4f7i5i1}
    \caption{}
    \label{fig:c4f9i5i1}
  \end{subfigure}
  \begin{subfigure}[t]{0.24\linewidth}
    \includegraphics[width=1\linewidth]{c4f7i5i2}
    \caption{}
   \label{fig:c4f9i5i2}
  \end{subfigure}
  \begin{subfigure}[t]{0.24\linewidth}
    \includegraphics[width=1\linewidth]{c4f7i5i3}
    \caption{}
   \label{fig:c4f9i5i3}
  \end{subfigure}
  \begin{subfigure}[t]{0.24\linewidth}
    \includegraphics[width=1\linewidth]{c4f7i5i3}
    \caption{}
   \label{fig:c4f9i5i4}
  \end{subfigure}
  
\caption{Effect of incorporating additional terms to the cost function. We used the \textit{Mansion} polygonal model (a), which was synthetically sampled to 14\,Mpts and used as input cloud. Color-coded normals are shown in (b) and color-coded sensor IDs (location from which each point was captured) are shown in (c). The color-coded local density deviation in the input is shown in (d).  
%
We first sub-sampled the cloud to 10\% using the unmodified cost function. Images (e) and (g) show bottom/top views of the resulting cloud. Rendering the cloud with normal culling, some gaps are apparent because the interior and exterior sides of some surfaces were processed jointly (in this model, walls were modeled with a single twoside surface sheet, with no thickness). We can avoid this by incorporating a normal-based weight to the cost function so that samples from different surface sides are ranked independently (f), (h). 
%
Image (i) shows the local density deviation on the original cloud. Images (j)-(l) also show density deviation on 10\% decimations  computed with different cost functions: original cost (j), using distances to the closest point on the same surface, based on normal agreement (k), and using the original cost but with a weight factor based on the normal variation on the neighborhood (l). 
Images (j)-(l) show that making the cost orientation-aware causes sample points to accumulate around feature edges.
We also explored adding a term to penalize samples with high expected range error (samples coming from a distant-oblique sensor). 
Image (m) shows the expected range error on the original cloud. The output with the unmodified cost function is shown in (n), whereas
(o) and (p) were computed by including a weight factor based on the scanner's range error. Notice that most red-colored points (high expected range error) have been removed from (o). A more aggressive simplification is shown in (p), where some red-colored points still survive, since inaccurate samples are removed only in sufficiently dense areas.} 
\label{fig:c4f9}
\end{figure}


==> figures/synthetic.tex <==

\begin{figure*}[!htb]
\centering
    %1
    %\includegraphics[width=0.16\linewidth]{synthetic/apartment_v10-10-1_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/apartment_v10-10-6_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/apartment_y00-10_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/apartment_y35-10_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/apartment_c10_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/apartment_d10_area.png}

    %2
    %\includegraphics[width=0.16\linewidth]{synthetic/baidinh_v10-10-1_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/baidinh_v10-10-6_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/baidinh_y00-10_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/baidinh_y35-10_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/baidinh_c10_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/baidinh_d10_area.png}
    
    %3
    %\includegraphics[width=0.16\linewidth]{synthetic/bungalow_v10-10-1_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/bungalow_v10-10-6_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/bungalow_y00-10_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/bungalow_y35-10_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/bungalow_c10_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/bungalow_d10_area.png}
    
    %4
    %\includegraphics[width=0.16\linewidth]{synthetic/cabin_v10-10-1_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/cabin_v10-10-6_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/cabin_y00-10_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/cabin_y35-10_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/cabin_c10_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/cabin_d10_area.png}
    
    %5
    \includegraphics[width=0.16\linewidth]{synthetic/cathedral_v10-10-1_area.png}
    \includegraphics[width=0.16\linewidth]{synthetic/cathedral_v10-10-6_area.png}
    \includegraphics[width=0.16\linewidth]{synthetic/cathedral_y00-10_area.png}
    \includegraphics[width=0.16\linewidth]{synthetic/cathedral_y35-10_area.png}
    \includegraphics[width=0.16\linewidth]{synthetic/cathedral_c10_area.png}
    \includegraphics[width=0.16\linewidth]{synthetic/cathedral_d10_area.png}
    
    %6
    %\includegraphics[width=0.16\linewidth]{synthetic/chapel_v10-10-1_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/chapel_v10-10-6_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/chapel_y00-10_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/chapel_y35-10_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/chapel_c10_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/chapel_d10_area.png}
    
    %7
    %\includegraphics[width=0.16\linewidth]{synthetic/church_v10-10-1_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/church_v10-10-6_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/church_y00-10_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/church_y35-10_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/church_c10_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/church_d10_area.png}
    
    %8
    \includegraphics[width=0.16\linewidth]{synthetic/cottage_v10-10-1_area.png}
    \includegraphics[width=0.16\linewidth]{synthetic/cottage_v10-10-6_area.png}
    \includegraphics[width=0.16\linewidth]{synthetic/cottage_y00-10_area.png}
    \includegraphics[width=0.16\linewidth]{synthetic/cottage_y35-10_area.png}
    \includegraphics[width=0.16\linewidth]{synthetic/cottage_c10_area.png}
    \includegraphics[width=0.16\linewidth]{synthetic/cottage_d10_area.png}
    
    %9
    \includegraphics[width=0.16\linewidth]{synthetic/highrise_v10-10-1_area.png}
    \includegraphics[width=0.16\linewidth]{synthetic/highrise_v10-10-6_area.png}
    \includegraphics[width=0.16\linewidth]{synthetic/highrise_y00-10_area.png}
    \includegraphics[width=0.16\linewidth]{synthetic/highrise_y35-10_area.png}
    \includegraphics[width=0.16\linewidth]{synthetic/highrise_c10_area.png}
    \includegraphics[width=0.16\linewidth]{synthetic/highrise_d10_area.png}
    
    %10
    %\includegraphics[width=0.16\linewidth]{synthetic/house_v10-10-1_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/house_v10-10-6_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/house_y00-10_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/house_y35-10_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/house_c10_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/house_d10_area.png}
    
    %11
    \includegraphics[width=0.16\linewidth]{synthetic/japanese_v10-10-1_area.png}
    \includegraphics[width=0.16\linewidth]{synthetic/japanese_v10-10-6_area.png}
    \includegraphics[width=0.16\linewidth]{synthetic/japanese_y00-10_area.png}
    \includegraphics[width=0.16\linewidth]{synthetic/japanese_y35-10_area.png}
    \includegraphics[width=0.16\linewidth]{synthetic/japanese_c10_area.png}
    \includegraphics[width=0.16\linewidth]{synthetic/japanese_d10_area.png}
    
    %12
    \includegraphics[width=0.16\linewidth]{synthetic/mansion_v10-10-1_area.png}
    \includegraphics[width=0.16\linewidth]{synthetic/mansion_v10-10-6_area.png}
    \includegraphics[width=0.16\linewidth]{synthetic/mansion_y00-10_area.png}
    \includegraphics[width=0.16\linewidth]{synthetic/mansion_y35-10_area.png}
    \includegraphics[width=0.16\linewidth]{synthetic/mansion_c10_area.png}
    \includegraphics[width=0.16\linewidth]{synthetic/mansion_d10_area.png}
    
    %13
    \includegraphics[width=0.16\linewidth]{synthetic/monastery_v10-10-1_area.png}
    \includegraphics[width=0.16\linewidth]{synthetic/monastery_v10-10-6_area.png}
    \includegraphics[width=0.16\linewidth]{synthetic/monastery_y00-10_area.png}
    \includegraphics[width=0.16\linewidth]{synthetic/monastery_y35-10_area.png}
    \includegraphics[width=0.16\linewidth]{synthetic/monastery_c10_area.png}
    \includegraphics[width=0.16\linewidth]{synthetic/monastery_d10_area.png}
    
    %14
    %\includegraphics[width=0.16\linewidth]{synthetic/mosque_v10-10-1_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/mosque_v10-10-6_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/mosque_y00-10_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/mosque_y35-10_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/mosque_c10_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/mosque_d10_area.png}
    
    %15
    \includegraphics[width=0.16\linewidth]{synthetic/oldhouse_v10-10-1_area.png}
    \includegraphics[width=0.16\linewidth]{synthetic/oldhouse_v10-10-6_area.png}
    \includegraphics[width=0.16\linewidth]{synthetic/oldhouse_y00-10_area.png}
    \includegraphics[width=0.16\linewidth]{synthetic/oldhouse_y35-10_area.png}
    \includegraphics[width=0.16\linewidth]{synthetic/oldhouse_c10_area.png}
    \includegraphics[width=0.16\linewidth]{synthetic/oldhouse_d10_area.png}
    
    %16
    %\includegraphics[width=0.16\linewidth]{synthetic/petersdom_v10-10-1_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/petersdom_v10-10-6_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/petersdom_y00-10_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/petersdom_y35-10_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/petersdom_c10_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/petersdom_d10_area.png}

    %17
    %\includegraphics[width=0.16\linewidth]{synthetic/pisa_v10-10-1_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/pisa_v10-10-6_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/pisa_y00-10_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/pisa_y35-10_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/pisa_c10_area.png}
    %\includegraphics[width=0.16\linewidth]{synthetic/pisa_d10_area.png}
    
    %18
    \includegraphics[width=0.16\linewidth]{synthetic/sanfrancisco_v10-10-1_area.png}
    \includegraphics[width=0.16\linewidth]{synthetic/sanfrancisco_v10-10-6_area.png}
    \includegraphics[width=0.16\linewidth]{synthetic/sanfrancisco_y00-10_area.png}
    \includegraphics[width=0.16\linewidth]{synthetic/sanfrancisco_y35-10_area.png}
    \includegraphics[width=0.16\linewidth]{synthetic/sanfrancisco_c10_area.png}
    \includegraphics[width=0.16\linewidth]{synthetic/sanfrancisco_d10_area.png}
\caption{}
\end{figure*}

